STEADY: Simultaneous State Estimation and Dynamics Learning from Indirect Observations

Accurate kinodynamic models play a crucial role in many robotics applications such as off-road navigation and high-speed driving. Many state-of-the-art approaches in learning stochastic kinodynamic models, however, require precise measurements of robot states as labeled input/output examples, which can be hard to obtain in outdoor settings due to limited sensor capabilities and the absence of ground truth. In this work, we propose a new technique for learning neural stochastic kinodynamic models from noisy and indirect observations by performing simultaneous state estimation and dynamics learning. The proposed technique iteratively improves the kinodynamic model in an expectation-maximization loop, where the E Step samples posterior state trajectories using particle filtering, and the M Step updates the dynamics to be more consistent with the sampled trajectories via stochastic gradient ascent. We evaluate our approach on both simulation and real-world benchmarks and compare it with several baseline techniques. Our approach not only achieves significantly higher accuracy but is also more robust to observation noise, thereby showing promise for boosting the performance of many other robotics applications.

==> STEADY Camera-ready arXiv/commands.tex <==
\newcommand{\algname}{STEADY}
\newcommand{\fixme}[1]{{\color{red} #1}}
\newcommand{\objective}{\Phi} % Optimization objective
\newcommand{\pair}[1]{\left\langle #1 \right\rangle}

\newcommand{\eg}{\textit{e.g.,}}
\newcommand{\etc}{\textit{etc.}}

\newcommand{\joydeep}[1]{\textcolor{red}{Joydeep:~#1}}

==> STEADY Camera-ready arXiv/sindy_related.tex <==
\section{Optimal Program Synthesis}
% mention SINDy and its limitation.
Our synthesis algorithm is largely inspired by the SINDy (\textbf{S}parse \textbf{I}dentification of \textbf{N}onlinear \textbf{Dy}namics) algorithm~\cite{brunton2016discovering}. The key insight behind SINDy is that many nonlinear dynamical systems can be written as a \emph{sparse} linear combination of only a few nonlinear terms, and therefore, they can be identified from data using sparsity-promiting linear regerssion techniques. For example, the famous Lorentz System can be written as 
\begin{align*}
  \dot{x} & = \sigma y - \sigma x \\
  \dot{y} & = \rho x - \rho y - z \\
  \dot{z} & = xy - \beta z\ ,
\end{align*}
where $\dot{x}$, $\dot{y}$, and $\dot{z}$ are the time derivatives of the states.
And if we choose the basis $\mathcal{B}$ to include all 3 state variables and their quadratic combinations, i.e., let $\mathcal{B} = [x, y, z, x^2, xy, xz, \ldots]$, we can then identify the correct dynamics using the collected state data $X$ and derivative data $\dot{X}$ by solving the following sparse linear regression problem
\begin{equation}
  \argmin_\Theta \Vert \mathcal{B}(X) \Theta - \dot{X} \Vert + \lambda \Vert \Theta \Vert_0\ , \label{eq:sindy-regression}
\end{equation}
where $\Theta$ is the coefficients matrix, $\Vert \Theta \Vert_0$ is the 0-norm that counts the number of nonzero entries in $\Theta$, and $\lambda$ controls the trad-off between sparsity and regression error.

\begin{figure}
  \begin{center}
  \includegraphics[width=0.45\linewidth]{images/sindy_model.png}
  \caption{The class of models identifiable by SINDy. The blue arrows on the right represent the sparse coefficients to be learned by the sparse linear regression algorithm.}
  \label{fig:sindy-model}
  \end{center}
\end{figure}

\begin{figure}
  \begin{center}
  \includegraphics[width=0.65\linewidth]{images/sedl_model.png}
  \caption{The class of models identifiable by \algname{}. Both the blue (middle) and red (right) arrows represent the sparse coefficients to be learned by the sparse nonlinear regression algorithm.}
  \label{fig:sedl-model}
  \end{center}
\end{figure}

From a machine learning perspective, we can view the class of models representable by SINDy as a sparsely linear layer with nonlinear input features, as shown in Figure~\ref{fig:sindy-model}. Although finding the optimal solution of \eqref{eq:sindy-regression} is generally NP-hard, recent analysis shows that the heuristics proposed in SINDy is very effective at finding the correct solutions in practice~\cite{zhang2019convergence}.


% 1d-car with dynamic friction.
However, in the class of robotics problems considered in this work, we found that the class of dynamics representable by SINDy is still too restrictive. For example, consider the dynamic friction forces of a 1-dimensional 2-wheel robot. The total friction has the form
\begin{align*}
  F_\mathrm{total} &= F_\mathrm{wheel,1} + F_\mathrm{wheel,2}\\
  &= f_1 \mathrm{sign}(r_1 \omega_1 - v) + f_2 \mathrm{sign}(r_2 \omega_2 - v)
\end{align*}
where $v$ is the robot's velocity, $\omega_1$ and $\omega_2$ are the angular velocities of the two wheels, $f_1, f_2, r_1, r_2$ are the parameters of the friction model, and the nonlinear function $\mathrm{sign}(x)$ is defined as $1$ if $x\geq0$ and $-1$ otherwise. Since the expressions inside the two $\mathrm{sign}$s are not simple state variables but involve unknown structures and parameters, we cannot use SINDy to identify this dynamics.

% Introduce our DSL and the synthesis algorithm.
Motivated by this, our synthesis algorithm generalizes the SINDy algorithm to target a larger class of dynamics of the form 
\begin{equation}
  \frac{dx}{dt} = \sum_{i=1}^N b_i \sigma_i\left(\sum_{j=1}^D a_{ij}v_j\right)\ , \label{eq:sedl-model}
\end{equation}
where $v_i$'s are elements from some basis $\mathcal{B}$ as in SINDy (e.g. state and control variables and their products), $\sigma_i$'s are parameter-free nonlinearities belonging to some library $\mathcal{F}$ (e.g. identity, sigmoid, sign, etc...), and $b_i$ and $a_{ij}$'s are the unknown and sparse coefficients to be identified. This dynamics form can be viewed as a two-layer neural network with sparse connections, as shown in Figure~\ref{fig:sedl-model}. If we include the identify function $\mathrm{id}$ in the library $\mathcal{F}$, then \eqref{eq:sedl-model} is a strict superset of the class of dynamics representable by SINDy.

\subsection{Synthesis with Nonlinear Sparse Regression}
Recall from Section~\ref{sec:problem-formulation} that our synthesis problem corresponds to solving the maximum likelihood estimation problem \eqref{eq:mle-problem} by searching the space of programs defined by our DSL. In SEDL, after taking the logritham of \eqref{eq:joint-likelihood} and discarding constant terms,  this corresponds to solving the following nonlinear sparse regression problem
\begin{equation}
  \argmin_{A, B, Q_\epsilon} \sum_{t=2}^T \log Q_{\epsilon}(x_t - f_{A, B}(x_{t-1}, u_t | x_t)), \label{eq:sedl-regression}
\end{equation}
where the states $x_t$ are obtained from the posterior sampling step \eqref{eq:posterior-sampling}, $A$ and $B$ are the collection of nonzero coefficients, and $f_{A,B}$ is the state derivatives given by the right-hand-side of \eqref{eq:sedl-model}. Since we only have finite amount of trajectory samples, to avoid overfitting, we apply the idea of cross validation~\cite{shao1993linear} by spliting our trajectory data into a training and validation set and using the performance on the validaton set to select the best model.

Like in SINDy, finding the optimal sparse solution to \eqref{eq:sedl-regression} is NP-hard, so we apply a greedy heuristic similar to the \emph{Stepwise sparse regression (SSR)} algorithm proposed in \cite{boninsegna2018sparse}. Our algorithm solves \eqref{eq:sedl-regression} iteratively, eliminating one coefficient at a time. Specifically, starting with all $N$ coefficients, there are $N$ ways to eliminate one of the coefficients, and our algorithm tries all $N$ ways and solve the corresponding optimization problems to get $N$ solutions. Then, the remaining $N-1$ coefficients that result in the highest performance are kept. By repeating this process until there is no coefficients left, we get a sequence of increasingly sparse solutions. Finally, we use the performance on the validation set to determine the best solution.


==> sindy_related.tex <==
\section{Optimal Program Synthesis}
% mention SINDy and its limitation.
Our synthesis algorithm is largely inspired by the SINDy (\textbf{S}parse \textbf{I}dentification of \textbf{N}onlinear \textbf{Dy}namics) algorithm~\cite{brunton2016discovering}. The key insight behind SINDy is that many nonlinear dynamical systems can be written as a \emph{sparse} linear combination of only a few nonlinear terms, and therefore, they can be identified from data using sparsity-promiting linear regerssion techniques. For example, the famous Lorentz System can be written as 
\begin{align*}
  \dot{x} & = \sigma y - \sigma x \\
  \dot{y} & = \rho x - \rho y - z \\
  \dot{z} & = xy - \beta z\ ,
\end{align*}
where $\dot{x}$, $\dot{y}$, and $\dot{z}$ are the time derivatives of the states.
And if we choose the basis $\mathcal{B}$ to include all 3 state variables and their quadratic combinations, i.e., let $\mathcal{B} = [x, y, z, x^2, xy, xz, \ldots]$, we can then identify the correct dynamics using the collected state data $X$ and derivative data $\dot{X}$ by solving the following sparse linear regression problem
\begin{equation}
  \argmin_\Theta \Vert \mathcal{B}(X) \Theta - \dot{X} \Vert + \lambda \Vert \Theta \Vert_0\ , \label{eq:sindy-regression}
\end{equation}
where $\Theta$ is the coefficients matrix, $\Vert \Theta \Vert_0$ is the 0-norm that counts the number of nonzero entries in $\Theta$, and $\lambda$ controls the trad-off between sparsity and regression error.

\begin{figure}
  \begin{center}
  \includegraphics[width=0.45\linewidth]{images/sindy_model.png}
  \caption{The class of models identifiable by SINDy. The blue arrows on the right represent the sparse coefficients to be learned by the sparse linear regression algorithm.}
  \label{fig:sindy-model}
  \end{center}
\end{figure}

\begin{figure}
  \begin{center}
  \includegraphics[width=0.65\linewidth]{images/sedl_model.png}
  \caption{The class of models identifiable by \algname{}. Both the blue (middle) and red (right) arrows represent the sparse coefficients to be learned by the sparse nonlinear regression algorithm.}
  \label{fig:sedl-model}
  \end{center}
\end{figure}

From a machine learning perspective, we can view the class of models representable by SINDy as a sparsely linear layer with nonlinear input features, as shown in Figure~\ref{fig:sindy-model}. Although finding the optimal solution of \eqref{eq:sindy-regression} is generally NP-hard, recent analysis shows that the heuristics proposed in SINDy is very effective at finding the correct solutions in practice~\cite{zhang2019convergence}.


% 1d-car with dynamic friction.
However, in the class of robotics problems considered in this work, we found that the class of dynamics representable by SINDy is still too restrictive. For example, consider the dynamic friction forces of a 1-dimensional 2-wheel robot. The total friction has the form
\begin{align*}
  F_\mathrm{total} &= F_\mathrm{wheel,1} + F_\mathrm{wheel,2}\\
  &= f_1 \mathrm{sign}(r_1 \omega_1 - v) + f_2 \mathrm{sign}(r_2 \omega_2 - v)
\end{align*}
where $v$ is the robot's velocity, $\omega_1$ and $\omega_2$ are the angular velocities of the two wheels, $f_1, f_2, r_1, r_2$ are the parameters of the friction model, and the nonlinear function $\mathrm{sign}(x)$ is defined as $1$ if $x\geq0$ and $-1$ otherwise. Since the expressions inside the two $\mathrm{sign}$s are not simple state variables but involve unknown structures and parameters, we cannot use SINDy to identify this dynamics.

% Introduce our DSL and the synthesis algorithm.
Motivated by this, our synthesis algorithm generalizes the SINDy algorithm to target a larger class of dynamics of the form 
\begin{equation}
  \frac{dx}{dt} = \sum_{i=1}^N b_i \sigma_i\left(\sum_{j=1}^D a_{ij}v_j\right)\ , \label{eq:sedl-model}
\end{equation}
where $v_i$'s are elements from some basis $\mathcal{B}$ as in SINDy (e.g. state and control variables and their products), $\sigma_i$'s are parameter-free nonlinearities belonging to some library $\mathcal{F}$ (e.g. identity, sigmoid, sign, etc...), and $b_i$ and $a_{ij}$'s are the unknown and sparse coefficients to be identified. This dynamics form can be viewed as a two-layer neural network with sparse connections, as shown in Figure~\ref{fig:sedl-model}. If we include the identify function $\mathrm{id}$ in the library $\mathcal{F}$, then \eqref{eq:sedl-model} is a strict superset of the class of dynamics representable by SINDy.

\subsection{Synthesis with Nonlinear Sparse Regression}
Recall from Section~\ref{sec:problem-formulation} that our synthesis problem corresponds to solving the maximum likelihood estimation problem \eqref{eq:mle-problem} by searching the space of programs defined by our DSL. In SEDL, after taking the logritham of \eqref{eq:joint-likelihood} and discarding constant terms,  this corresponds to solving the following nonlinear sparse regression problem
\begin{equation}
  \argmin_{A, B, Q_\epsilon} \sum_{t=2}^T \log Q_{\epsilon}(x_t - f_{A, B}(x_{t-1}, u_t | x_t)), \label{eq:sedl-regression}
\end{equation}
where the states $x_t$ are obtained from the posterior sampling step \eqref{eq:posterior-sampling}, $A$ and $B$ are the collection of nonzero coefficients, and $f_{A,B}$ is the state derivatives given by the right-hand-side of \eqref{eq:sedl-model}. Since we only have finite amount of trajectory samples, to avoid overfitting, we apply the idea of cross validation~\cite{shao1993linear} by spliting our trajectory data into a training and validation set and using the performance on the validaton set to select the best model.

Like in SINDy, finding the optimal sparse solution to \eqref{eq:sedl-regression} is NP-hard, so we apply a greedy heuristic similar to the \emph{Stepwise sparse regression (SSR)} algorithm proposed in \cite{boninsegna2018sparse}. Our algorithm solves \eqref{eq:sedl-regression} iteratively, eliminating one coefficient at a time. Specifically, starting with all $N$ coefficients, there are $N$ ways to eliminate one of the coefficients, and our algorithm tries all $N$ ways and solve the corresponding optimization problems to get $N$ solutions. Then, the remaining $N-1$ coefficients that result in the highest performance are kept. By repeating this process until there is no coefficients left, we get a sequence of increasingly sparse solutions. Finally, we use the performance on the validation set to determine the best solution.

